QFuzz: Quantitative Fuzzing for Side Channels

Side channels pose a significant threat to the confidentiality of software systems. Such vulnerabilities are challenging to detect and evaluate because they arise from non-functional properties of software such as execution times and require reasoning on multiple execution traces. Recently, noninterference notions have been adapted in static analysis, symbolic execution, and greybox fuzzing techniques. However, noninterference is a strict notion and may reject security even if the strength of information leaks are weak. A quantitative notion of security allows for the relaxation of noninterference and tolerates small (unavoidable) leaks. Despite progress in recent years, the existing quantitative approaches have scalability limitations in practice. In this work, we present QFuzz, a greybox fuzzing technique to quantitatively evaluate the strength of side channels with a focus on min entropy. Min entropy is a measure based on the number of distinguishable observations (partitions) to assess the resulting threat from an attacker who tries to compromise secrets in one try. We develop a novel greybox fuzzing equipped with two partitioning algorithms that try to maximize the number of distinguishable observations and the cost differences between them. We evaluate QFuzz on a large set of benchmarks from existing work and real-world libraries (with a total of 70 subjects). QFuzz compares favorably to three state-of-the-art detection techniques. QFuzz provides quantitative information about leaks beyond the capabilities of all three techniques. Crucially, we compare QFuzz to a state-of-the-art quantification tool and find that QFuzz significantly outperforms the tool in scalability while maintaining similar precision. Overall, we find that our approach scales well for real-world applications and provides useful information to evaluate resulting threats. Additionally, QFuzz identifies a zero-d...

==> Makefile <==
# NOTE: you must install latexmk first!!

LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

MAIN=main
SOURCES=$(MAIN).tex Makefile header.tex introduction.tex overview.tex Overview-code.tex definition.tex approach.tex greedyAlgo.tex experiments.tex table-clustering.tex table-blazer.tex table-diffuzz.tex table-rsa.tex table-themis.tex implementation.tex related-work.tex limitation.tex conclusion.tex papers.bib
FIGURES=
#FIGURES := $(shell find figures/* images/* -type f)

all:    $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) \
	-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

online: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
	-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk *.refresh *.DS_Store

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all


==> implementation.tex <==
\stsays{we need to provide our implementation approach here!}

(1) implementation of $Clust$ algorithm!

(2) Explanation how we set $\epsilon$ value.

(3) Upper-bound $K$. If we run fuzzer for certain amounts of times, and found $K$
clusters, is it possible to stop, change $K$ to $2*K$, and run the fuzzer again
such that it uses the inputs from the previous run?

\ynsays{K is given to the fuzzer? It would be something like a maximum input length.
This means we only can find up to K different clusters. We could also try to make
K dynamic, i.e. it is part of the input, but this is maybe not feasible.
We can first start with a constant K and try different values.}

\stsays{Yeah, exactly. We can start by having a constant value for K
as an upper-bound. The fuzzer may find K cluster or less in this case.
The dynamic idea is applicable if the fuzzer finds $K$ different clusters
in the given time limit and we can somehow? modify the driver to look for $K+1$
cluster!}


(4) To obtain the minimum distance $\delta$ among clusters, we first
calculate the minimum and maximum costs in each class of observation.
Then, we compare the maximum cost of one cluster to the minimum
cost of another cluster. We pick the smallest positive cost differences
as the value of $\delta$.

\ynsays{I just wanted to write down some ideas on how to implement this with DifFuzz.}

At the moment DifFuzz~\cite{DBLP:conf/icse/nilizadeh} stores a cost difference highscore internally in the fuzzer.
This cost difference highscore represents the maximum cost difference observed so far for the same public input and different secret inputs.
The goal, in order to identify potential side-channels, was to maximize this cost difference.

For our approach we need to change this cost function because we would like to find all possible different secret values.

The driver in DifFuzz fuzzes three values: one public value and two secret values.
Our driver needs to fuzz K+1 values: one public value, and K secret values.
The driver in DifFuzz assess the values by comparing their cost values and tells the fuzzer to keep the inputs if they maximized the highscore.
Our driver needs to assess the values also by comparing their cost values, but it will also count the number of \textit{distinguishable} observations.
Our highscore will be the number of \textit{distinguishable} observations.

(6) About the extension to $m$ trials. \stsays{I will try to include
preliminary results on simple programs, but will say that: In this paper,
however, we only focus on the threat model with
a single public input and left the further analysis for threat models
with multiple trials and its connections to adaptive side channels
as future work.}


==> micro-benchmark.tex <==
Here, we include micro-benchmark

